Geography of the cubic connectedness locus I: Intertwining surgery

We exhibit products of Mandelbrot sets in the two-dimensional complex parameter space of cubic polynomials. These products were observed by J. Milnor in computer experiments which inspired Lavaurs' proof of non local-connectivity for the cubic connectedness locus. Cubic polynomials in such a product may be renormalized to produce a pair of quadratic maps. The inverse construction is an {\it intertwining surgery} on two quadratics. The idea of intertwining first appeared in a collection of problems edited by Bielefeld. Using quasiconformal surgery techniques of Branner and Douady, we show that any two quadratics may be intertwined to obtain a cubic polynomial. The proof of continuity in our two-parameter setting requires further considerations involving ray combinatorics and a pullback argument.

==> mycyr.tex <==
%auto-ignore
\catcode`\@=11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% University of Washington cyrillic family
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{UWCyr}{m}{n}{%
   <5>wncyr5%
   <6>wncyr6%
   <7>wncyr7%
   <8>wncyr8%
   <9>wncyr9%
   <10>wncyr10%
   <11>wncyr10 at10.95pt%
   <12>wncyr10 at12pt%
   <14>wncyr10 at14.4pt%
   <17>wncyr10 at17.28pt%
   <20>wncyr10 at20.74pt%
   <25>wncyr10 at24.88pt}{}

\new@fontshape{UWCyr}{m}{it}{%
   <5>wncyi5%
   <6>wncyi6%
   <7>wncyi7%
   <8>wncyi8%
   <9>wncyi9%
   <10>wncyi10%
   <11>wncyi10 at10.95pt%
   <12>wncyi10 at12pt%
   <14>wncyi10 at14.4pt%
   <17>wncyi10 at17.28pt%
   <20>wncyi10 at20.74pt%
   <25>wncyi10 at24.88pt}{}

\new@fontshape{UWCyr}{m}{sc}{%
   <5>wncysc10 at5pt%
   <6>wncysc10 at6pt%
   <7>wncysc10 at7pt%
   <8>wncysc10 at8pt%
   <9>wncysc10 at9pt%
   <10>wncysc10%
   <11>wncysc10 at10.95pt%
   <12>wncysc10 at12pt%
   <14>wncysc10 at14.4pt%
   <17>wncysc10 at17.28pt%
   <20>wncysc10 at20.74pt%
   <25>wncysc10 at24.88pt}{}

%%%%%%%%%%%%% bold series

\new@fontshape{UWCyr}{b}{n}{%
   <5>wncyb5%
   <6>wncyb6%
   <7>wncyb7%
   <8>wncyb8%
   <9>wncyb9%
   <10>wncyb10%
   <11>wncyb10 at10.95pt%
   <12>wncyb10 at12pt%
   <14>wncyb10 at14.4pt%
   <17>wncyb10 at17.28pt%
   <20>wncyb10 at20.74pt%
   <25>wncyb10 at24.88pt}{}

\extra@def{UWCyr}{}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% University of Washington cyrillic sans serif family
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\new@fontshape{UWCyss}{m}{n}{%
   <5>wncyss8 at5pt%
   <6>wncyss8 at6pt%
   <7>wncyss8 at7pt%
   <8>wncyss8%
   <9>wncyss9%
   <10>wncyss10%
   <11>wncyss10 at10.95pt%
   <12>wncyss10 at12pt%
   <14>wncyss10 at14.4pt%
   <17>wncyss10 at17.28pt%
   <20>wncyss10 at20.74pt%
   <25>wncyss10 at24.88pt}{}

\extra@def{UWCyss}{}{}

\catcode`\@=\active


==> proofs.tex <==
%auto-ignore
\section{Proof of the Main Theorem}
\label{proofs}


\begin{prop} \label{proper}
$\lrren:B_{p/q,m}\to(\M\setminus\{\rt\})\times(\M\setminus\{\rt\})$
is proper.
\end{prop}

\smallskip
In view of the compactness of the connectedness loci, it
suffices to prove that if $(A_k,D_k)\in B_{p/q,m}$ with
$$(A_k,D_k)\to(A_\infty,D_\infty)\in \CubM\;\;\mbox{ and }\;\;
\lrren(A_k,D_k)\to(c_\infty,\tl c_\infty)\in \M\times\M$$
then $(A_\infty,D_\infty)
\in B_{p/q,m}$ if and only if $c_\infty\neq\rt\neq\tl c_\infty$.
We require an auxiliary lemma and some further notation.
Let $\zeta_k$ be the unique repelling fixed point of $P_k=P_{A_k,D_k}$
where $2q$ external rays land, and let $\zeta_k^-$ and $\zeta_k^+$ be
the points of period $q$ which renormalize to $\alpha_{f_{c_k}}$
and $\alpha_{f_{\tl c_k}}$. We write $\mu_k$ and $\mu^\pm_k$ for the
multipliers of $\zeta_k$ and $\zeta^\pm_k$, and $\lambda_k^\pm$ for the
multipliers of the corresponding $\alpha$-fixed points. 
Passing to a subsequence if necessary, we may assume without loss of
generality that the $\zeta_k$ converge to a fixed point $\zeta_\infty$
of $P_\infty=P_{A_\infty,D_\infty}$ with multiplier $\mu_\infty$,
and the $\zeta_k^\pm$ converge to periodic points $\zeta^\pm_\infty$ with
multipliers $\mu^\pm_\infty$.

\begin{lem}
\label{stays-repelling}
In this setting, if $c_\infty\neq\rt\neq\tl c_\infty$ then 
$\zeta^{-}_\infty$, $\zeta_\infty$ and $\zeta^{+}_\infty$ belong to 
disjoint orbits. Moreover, the fixed point $\zeta_\infty$ is repelling.
\end{lem}

\begin{pf}
It follows from the Implicit Function Theorem that these orbits are
distinct unless one of $\zeta^\pm_\infty$ is parabolic with multiplier 1.
Without loss of generality $\mu_\infty^-=1$, and we may further assume 
that either $|\mu^-_k|\leq 1$ for every $k$ or $|\mu^-_k|>1$ for every
$k$. In the first case, $\lambda^-_k=\mu^-_k$ by Remark \ref{eigrmk}, 
and $\lambda^-_k\to 1$ implies $c=\rt$. In the second case, it similarly 
follows that $|\lambda^-_k|>1$ for every $k$; in view of Yoccoz Inequality, 
$c_k\in L_{p_k/q_k}$ where $p_k/q_k\to 0$, whence
$\lambda^-_k\to 1$ and again $c=\rt$. 

Because $\zeta_\infty^-$, $\zeta_\infty$ and $\zeta^\pm_
\infty$ lie in distinct orbits, it follows from Kiwi's
Separation \lemref{separation} that at least one of these points is repelling.
Suppose first that $\zeta^-_\infty$ is repelling, and let $\gamma^-_k
\in K(P_k)$ be the points which renormalize to
$-\alpha_{f_{c_k}}\in K(f_{c_k})$. Then $\gamma^-_k\to\gamma^-_\infty$
where $P_\infty(\gamma^-_\infty)=\zeta^-_\infty$, and 
the rays landing at $\gamma^-_\infty$ separate $\zeta_\infty$ from the
critical point $-1$. Similarly, if $\zeta^+_\infty$
is repelling then the rays landing at the corresponding point
$\gamma^+_\infty$ separate $\zeta_\infty$ from $+1$. 
Applying \lemref{separation} once again, we conclude that $\zeta_\infty$ is
repelling.
\end{pf}

Continuing with the proof of \propref{proper}, we observe by
\lemref{same-rays} that $\zeta_\infty$ is the common landing point of
the same two cycles of rays with rotation number $p/q$.
The thickening procedure yields a pair of quadratic-like restrictions
$$P_\infty^{\circ q}:\Omega_\infty'\to \Omega_\infty\;\;
\n\;\; P_\infty^{\circ q}:\tl\Omega_\infty'\to\tl\Omega_\infty,$$
and we may arrange for $\Omega'_\infty$ and $\tl\Omega'
_\infty$ to be the limits of thickened domains $\Omega'_k$ and $\tl\Omega'_k$
for the quadratic-like restrictions of $P^{\circ q}_k$. As 
$P_k^{\circ qn}(-1)\in \Omega'_k$ and $P_k^{\circ qn}(+1)\in \tl\Omega'_k$,
it follows that $P_\infty^{\circ qn}(-1)\in\Omega'_\infty$ and $P_\infty^
{\circ qn}(+1)\in\tl\Omega'_\infty$. Thus, $P_\infty$ is birenormalizable,
that is, $(A_\infty,D_\infty)\in B_{p/q,m}$. $\;\;\Box$

\bigskip
Setting $$h_{p/q.m}(c,\tl c)=(\lrren)^{-1}(\kappa_{p/q}(c),
\kappa_{p/q}(\tl c))$$
so that
$h_{p/q,m}(c,\tl c)=(A,D)$ if and only if  $P_{A,D}=f_c
{\underset{p/q,m}{\intr}} f_{\tl c}$
we obtain the embeddings
$$h_{p/q,m}:(\M_{p/q}\setminus\{\rt_{p/q}\})\times(\M_{p/q}\setminus
\{\rt_{p/q}\})\longrightarrow B_{p/q,m}\subset C_{p/q,m}$$
whose existence was asserted in \thmref{main}.
As observed in \secref{outline}, if $P=P_{A,D}$ is birenormalizable
and $(A,D)\in\CubMR$ then $p/q=0$ or $1/2$. It follows by symmetry that 
$\lrren(A,D)=(c,\bar c)$ for some $c\in\BBB C$; conversely, if
$\lrren(A,D)=(c,\bar c)$ then $(A,D)\in\CubMR$.
Writing $\bar\Delta$ for the antidiagonal
embedding $\BBB C\ni c\mapsto(c,\bar c)\in{\BBB C}^2$, we define
$$\Psi_{1/2,1}= h_{1/2,1}\circ \bar\Delta
:\M_{1/2}\setminus\{\rt_{1/2}\}\to\CubMR\cap C_{1/2,1}$$
$$\Psi_{1/2,3}= h_{1/2,3}\circ \bar\Delta
:\M_{1/2}\setminus\{\rt_{1/2}\}\to\CubMR\cap C_{1/2,3}$$
and
$$\Psi_0= h_0\circ \bar\Delta:\M\setminus\{\rt\}\to\CubMR\cap C_0.$$
These are the embeddings whose existence was asserted
in \thmref{real-main-thm}. Compatibility with the standard
planar embeddings is a consequence of the following recent result of
Buff \cite{Buff}:

\begin{thm}
\label{ext}
Let $K_1$ and $K_2$ be compact, connected, cellular sets in the plane, and
$\varphi:K_1\to K_2$ a homeomorphism. If $\varphi$ admits a continuous
extension to an open neighborhood of $K_1$ such that points outside $K_1$
map to points outside $K_2$, then $\varphi$ extends to a homeomorphism
between open neighborhoods of $K_1$ and $K_2$. 
\end{thm}

Let us sketch the argument for the map $\Psi_0$. It is easily verified from
the explicit expressions in \cite[p. 22]{Mil} that for each $\mu\in{\BBB C}
\setminus\{1\}$ there is a unique pair $(A,B)\in\BBB R^2$ such that the
corresponding polynomial in the normal form (\ref{normal-form}) has a pair of
complex conjugate fixed points with multipliers $\mu$ and $\bar\mu$, the
remaining fixed point having eigenvalue
$$\nu=1+\frac{|\mu-1|^2}{2\Re(\mu-1)}.$$ 
We may continuously label these multipliers as $\mu(A,D)$, $\bar\mu(A,D)$
and $\nu(A,D)$ for parameter values $(A,D)\in\BBB R\times i\BBB R$
in a neighborhood of $\Psi_0(\M\setminus\{\rt\})$;
in particular, $(A,D)\mapsto\mu(A,D)$ is a homeomorphism on such a 
neighborhood. It follows from Yoccoz Inequality (\ref{yoccoz}) that
$\nu(A,D)>1$, and therefore $\mu(A,D)\not\in[1,\infty)$, for $(A,D)$ in 
$\Psi_0(\M\setminus\{\rt\})$. Similarly, $\mu(\Psi_0(c))\to 1$ as 
$c\to\rt$, and thus $c\mapsto\mu(\Psi_0(c))$ extends to a embedding
$$\Upsilon:\M\to \BBB C\setminus(1,\infty)$$ which clearly commutes
with complex conjugation.

We claim that $\Upsilon^{-1}:\Upsilon(\M)\to \M$
admits a continuous extension meeting the condition of \thmref{ext}.
The idea is to allow renormalizations with disconnected Julia sets.
Recalling \lemref{same-rays}, we note that
the rays $r_0$ and $r_{1/2}$ continue to land at the same fixed point
for $(A,D)$ in a neighborhood of $\Psi_0(\M\setminus\{\rt\})$. 
As before, we may construct left and right quadratic-like restrictions 
with continuously varying domains $\Omega'_{A,D}$.
It is emphasized in Douady and Hubbard's
original presentation \cite{DH} that straightening, while no longer canonical
for maps with disconnected Julia set, may still be continuously defined: 
it is only necessary to begin with continuously varying 
quasiconformal homeomorphisms from the fundamental annuli 
$\Omega_{A,D}\setminus\Omega'_{A,D}$ to the standard annulus. We
thereby obtain a continuous extension to a neighborhood of
$\Upsilon(\M\setminus\{\rt\})$; it is easily arranged that this extension
commutes with complex conjugation, so that it is trivial to obtain a
further extension to an open set containing the point $1$.










